Non-Hermitian Gravitational Wave Scattering

In this study, the non-Hermitian scattering of gravitational waves is examined, and their behavior at spectral singularities is discussed. We investigate the non-Hermitian properties of gravitational waves through the construction of a transfer matrix. By examining spectral singularity points obtained from the transfer matrix, we explore the behavior of gravitational waves at these spectral singularity points and compare the theoretical results with observed measurements. Our findings demonstrate that the frequency values of gravitational waves measured on Earth at spectral singularity points exhibit perfect agreement with the corresponding Hubble constant values. This alignment underscores the significance of the non-Hermitian characteristics of gravitational waves. We anticipate that this research will contribute to a deeper understanding of the role of non-Hermitian phenomena in gravitational physics and provide a foundation for future studies in the field.

==> diff.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Welcome to Overleaf --- just edit your LaTeX on the left,
% and we'll compile it for you on the right. If you open the
% 'Share' menu, you can invite other users to edit at the same
% time. See www.overleaf.com/learn for more info. Enjoy!
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\RequirePackage{shellesc}
%\ShellEscape{latexdiff Burak.tex R1-Burak.tex > main-d.tex}
%\input{main-d}
%\documentclass{dummy}
%\title{Demonstrating latexdiff}
